Structured Query Reformulations in Commerce Search

Recent work in commerce search has shown that understanding the semantics in user queries enables more effective query analysis and retrieval of relevant products. However, due to lack of sufficient domain knowledge, user queries often include terms that cannot be mapped directly to any product attribute. For example, a user looking for {\tt designer handbags} might start with such a query because she is not familiar with the manufacturers, the price ranges, and/or the material that gives a handbag designer appeal. Current commerce search engines treat terms such as {\tt designer} as keywords and attempt to match them to contents such as product reviews and product descriptions, often resulting in poor user experience. In this study, we propose to address this problem by reformulating queries involving terms such as {\tt designer}, which we call \emph{modifiers}, to queries that specify precise product attributes. We learn to rewrite the modifiers to attribute values by analyzing user behavior and leveraging structured data sources such as the product catalog that serves the queries. We first produce a probabilistic mapping between the modifiers and attribute values based on user behavioral data. These initial associations are then used to retrieve products from the catalog, over which we infer sets of attribute values that best describe the semantics of the modifiers. We evaluate the effectiveness of our approach based on a comprehensive Mechanical Turk study. We find that users agree with the attribute values selected by our approach in about 95% of the cases and they prefer the results surfaced for our reformulated queries to ones for the original queries in 87% of the time.

==> algorithm.tex <==
\section{The Algorithm}

Let us first consider the following simple algorithm. 
From the set of browse trails, we initially compute
the values of $f_{qp}$ for each $p\in P, q\in Q$.
By our assumption, 
\begin{equation*} 
f_{qp} \geq \alpha\left(\frac{s_{qq'}n_q}{m_{q'}}\right),
\end{equation*}
where $q' = I(p)$.
Further, by the $\beta$-proportionality assumption, we know
that for any $p\in P_q$,
\begin{eqnarray*}
f_{qp} & \geq & \alpha\left(\frac{s_{qq}n_q}{m_q}\right)\\
f_{qp}& \geq & \alpha\beta s_{qq}\left(\frac{n}{m}\right)\\
f_{qp}\left(\frac{m}{n}\right) & \geq & \alpha\beta s_{qq}.
\end{eqnarray*}
Let us define $g_{qp} = f_{qp}\left(\frac{m}{n}\right)$.
If $s_{qq}\geq \theta$, then
\begin{equation*}
g_{qp} \geq \alpha\beta\theta.
\end{equation*}
$g_{qp}$ is known; let us assume that 
the values of $\alpha$ and $\beta$ are known as well.\footnote{
The values of $\alpha$ and $\beta$ can be estimated using training
data.} Then, 
we can compute $g_{qp}$ for each page $p$, and keyword $q$, 
and retain all those keywords such that 
$g_{qp}\geq \alpha\beta\theta$.

Let us try to estimate the size of the lists we create using
the above algorithm. 
\begin{theorem}\label{thm:size}
The sum of the length of the lists for all the pages is 
$\left(\frac{\gamma}{\alpha\beta\theta}\right)m$.
\end{theorem}
\begin{proof}
\begin{eqnarray*}
g_{qp} & = & f_{qp}\left(\frac{m}{n}\right)\\
\Rightarrow \sum_{p\in P} g_{qp} & = & \left(\frac{m}{n}\right)\sum_{p\in P}f_{qp}\\
& = & \left(\frac{m}{n}\right)n_q\\
& \leq & \gamma m_q.
\end{eqnarray*}
Thus, a keyword $q$ can feature in at most 
$\frac{\gamma m_q}{\alpha\beta\theta}$ lists. Therefore, the sum
of length of the lists is at most
\begin{equation*}
\sum_{q\in Q}\frac{\gamma m_q}{\alpha\beta\theta} = \left(\frac{\gamma}{\alpha\beta\theta}\right)m.
\end{equation*}
Thus, there is a space overhead factor of 
$\frac{\gamma}{\alpha\beta\theta}$.
\end{proof}

Let $L_p$ be the list of keywords produced for page $p$
by the above algorithm. One shortcoming of the above
algorithm is that we get no guarantees about the
composition of $L_p$, other than the fact that 
$q = I(p)\in L_p$ if $s_{qq}\geq \theta$. We now modify
the above algorithm to provide guarantees about the
composition of $L_p$. Since $n_q$ is known, we can compute 
$h_{qp} = g_{qp}/n_q$. Let $H = \max_{q\in Q} h_{qp}$. We
compute $h_{qp}' = h_{qp}/H$ and include those $q$
in list $L_p'$ which have 
$h_{qp}'\geq \frac{\alpha\beta\theta}{\gamma\delta}$. 

We first prove that $L_p'$ contains $I(p)$ if 
$s_{qq}\geq \theta$.
\begin{theorem}\label{thm:correctness-2}
Each keyword $q$ with
$s_{qq}\geq \theta$ is included in $L'_p$ for each 
$p\in P_q$.
\end{theorem}
\begin{proof}
If $q = I(p)$ for a page $p$ and $q'$ is any keyword,
\begin{equation}\label{eq:h-bound}
\alpha\beta\left(\frac{s_{q'q}}{n_q}\right)\leq h_{q'p}\leq \gamma\delta\left(\frac{s_{q'q}}{n_q}\right),
\end{equation}. We know that
$s_{qq}\geq \theta$; hence,
\begin{equation}\label{eq:H-bound}
\alpha\beta\left(\frac{\theta}{n_q}\right)\leq H
\leq \gamma\delta\left(\frac{1}{n_q}\right).
\end{equation}
Hence,
\begin{equation*}
h_{qp}' \geq \frac{\alpha\beta\theta}{\gamma\delta}.
\end{equation*}
\end{proof}

Now, we prove that keywords $q'$ with very small values
of $s_{q'q}$ are not included in the list $L_p'$ for any
$p\in P_q$.
\begin{theorem}\label{thm:errorbound-2}
If $q'\in L_p'$, where $I(p) = q$, then 
\begin{equation*}
s_{q'q}\geq \left(\frac{\alpha\beta\theta}{\gamma\delta}\right)^2.
\end{equation*}
\end{theorem}
\begin{proof}
From Eqns.~\ref{eq:h-bound} and \ref{eq:H-bound}, we have
\begin{equation*}
h_{q'p}' \leq \left(\frac{\gamma\delta}{\alpha\beta\theta}\right)s_{q'q}.
\end{equation*}
If $h_{q'p}'\geq \frac{\alpha\beta\theta}{\gamma\delta}$, then
\begin{equation*}
s_{q'q}\geq \left(\frac{\alpha\beta\theta}{\gamma\delta}\right)^2.
\end{equation*}
\end{proof}

The final step in our algorithm is taking the intersection of $L_p$
and $L_p'$ to create the final list of keywords for page $p$. Clearly,
this retains both the correctness property (demonstrated in both sets
of lists) and the size bounds (demonstrated in the $L_p$ lists).

\subsection{Algorithm in the Streaming Model}

In reality, the algorithm does not get the function $f$ as input,
rather it gets (keyword, page) pairs $(q, p)$, where it is infeasible
to compute the function $f_{qp}$ for each $q\in Q, p\in P$. Thus, 
we need to port the above algorithm to the data streaming model.
The key observation is that the algorithm above essentially uses 
(possibly scaled) frequency counts. Let us first consider the 
construction of the lists $L_p$. Recall that the algorithm seeks
to populate the list $L_p$ with keywords $q$ such that 
$f_{qp}\geq \frac{\alpha\beta\theta n}{m}$. For this purpose,
we use a standard heavy hitters algorithm~\ref{heavy-hitters}. 
We maintain a list 
$\cal L$ of $\frac{m}{S\alpha\beta\theta}$ 
(keyword, page) pairs $(q, p)$ and their frequencies $f'(q, p)$, 
for some parameter $S < 1$. When a new (keyword, page) pair 
$(q, p)$ appears on the data stream, we update $\cal L$ as follows:
\begin{itemize} 
\item if $(q, p)\in {\cal L}$ , increase $f'(q, p)$ by 1,
\item otherwise, if $\cal L$ is not full, insert $(q, p)$ into $\cal L$
and set $f(q, p) = 1$,
\item otherwise, decrease $f(q', p')$ for each entry $(q', p')$ in 
$\cal L$ by 1, and remove an entry if its frequency becomes 0.
\end{itemize}
The following theorem is standard in the streaming literature.
\begin{theorem}\label{thm:freq}
All $(q, p)$ pairs with
$f_{qp}\geq \frac{\alpha\beta\theta n}{m}$ are retained in $\cal L$, 
and have 
\begin{equation*}
f'(q, p)\geq (1-S)\left(\frac{\alpha\beta\theta n}{m}\right).
\end{equation*}
\end{theorem}
Finally, we remove all the (query, keyword) pairs $(q, p)$ with 
$f'(q, p) < (1-S)\left(\frac{\alpha\beta\theta n}{m}\right)$.
Extending the proof of Theorem~\ref{thm:size}, we get the following
theorem.
\begin{theorem}
The sum of the length of the lists for all the pages created by
the above algorithm is at most
$\left(\frac{\gamma}{(1-S)\alpha\beta\theta}\right)m$.
\end{theorem}

We now need to construct the lists $L_p'$. We use 
Theorem~\ref{thm:freq} for this purpose. We use the algorithm
in the static model described earlier, using $f'(q, p)$ 
for $f_{qp}$, except that in the last step, we include all 
$q$ for page $p$ which have 
\begin{equation*}
h_{qp}'\geq \frac{(1-S)\alpha\beta\theta}{\gamma\delta}.
\end{equation*}
Theorem~\ref{thm:correctness-2} continues to hold for the new
algorithm. However, Theorem~\ref{thm:errorbound-2} has to be modified
slightly to the following theorem.
\begin{theorem}\label{thm:errorbound-3}
If $q'\in L_p'$, where $I(p) = q$, then 
\begin{equation*}
s_{q'q}\geq \left(\frac{(1-S)\alpha\beta\theta}{\gamma\delta}\right)^2.
\end{equation*}
\end{theorem}
